Predicted Composite Signed-Distance Fields for Real-Time Motion Planning in Dynamic Environments

We present a novel framework for motion planning in dynamic environments that accounts for the predicted trajectories of moving objects in the scene. We explore the use of composite signed-distance fields in motion planning and detail how they can be used to generate signed-distance fields (SDFs) in real-time to incorporate predicted obstacle motions. We benchmark our approach of using composite SDFs against performing exact SDF calculations on the workspace occupancy grid. Our proposed technique generates predictions substantially faster and typically exhibits an 81--97% reduction in time for subsequent predictions. We integrate our framework with GPMP2 to demonstrate a full implementation of our approach in real-time, enabling a 7-DoF Panda arm to smoothly avoid a moving robot.

==> figures/fig-curved-traj-heatmap.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/images/curved_collision_heatmap.png}
    \caption{Stress-test results for the constant-velocity model. Dark blue cells indicate that the executed trajectory resulted in collision. 
    %  across a range of curved trajectories (determined by the radius) and obstacle speeds
    % The constant-velocity is robust when the obstacle speed is low for a given curvature path, relative to the update frequency of the tracker.
    }
    \label{fig:curved_traj_heatmap}
\end{figure}

==> figures/fig-profiling.tex <==
\begin{figure}
    \centering
        \includegraphics[width=1.0\columnwidth]{figures/images/matlab_profiling.png}
    \caption{MATLAB code profiling for the first iteration of the update loop (averaged over ten trials). A significant amount of time is spent on publishing the resultant trajectory and re-formatting the signed-distance fields for use in the GPMP2 data structure; we believe that these time costs could be further optimised by moving to a `non-MATLAB' implementation and initialising the SDF structure in parallel.}
    \label{fig:profiling}
\end{figure}
